Training Robots to Evaluate Robots: Example-Based Interactive Reward Functions for Policy Learning

Physical interactions can often help reveal information that is not readily apparent. For example, we may tug at a table leg to evaluate whether it is built well, or turn a water bottle upside down to check that it is watertight. We propose to train robots to acquire such interactive behaviors automatically, for the purpose of evaluating the result of an attempted robotic skill execution. These evaluations in turn serve as "interactive reward functions" (IRFs) for training reinforcement learning policies to perform the target skill, such as screwing the table leg tightly. In addition, even after task policies are fully trained, IRFs can serve as verification mechanisms that improve online task execution. For any given task, our IRFs can be conveniently trained using only examples of successful outcomes, and no further specification is needed to train the task policy thereafter. In our evaluations on door locking and weighted block stacking in simulation, and screw tightening on a real robot, IRFs enable large performance improvements, even outperforming baselines with access to demonstrations or carefully engineered rewards. Project website: https://sites.google.com/view/lirf-corl-2022/

==> algos/fsm_algo.tex <==
\begin{algorithm}[h]
\small
\caption{LIRF+Verify Pseudocode}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Require:}}
% \REQUIRE single-observation reward classifier $D(o) \rightarrow [0, 1]$, positive actionable examples $P$.
\REQUIRE LIRF policy $\pi_T$, IRF policy $\pi_R$, single-observation reward $D(o) \rightarrow [0, 1]$
\STATE $i = 0$
\STATE Rollout $\pi_T$ in the task POMDP.
\STATE Keep the world state, switch to IRF POMDP and rollout $\pi_R$. The final observation is $o^*$.
\STATE $i{+}{+}$
\IF {$D(o^*) > 0.5$ or $i \geq 10$}
    \STATE Terminate
\ELSE
    \STATE Keep the world state, repeat from 1.
\ENDIF

\end{algorithmic}
\label{algo:main_algo_expanded}

\end{algorithm}

% \setlength{\floatsep}{0.1cm}


==> algos/supp_algo_w_math.tex <==
% \hk{VICE or simply classifier-based rewards?}
\begin{algorithm}[t]
\caption{Adversarial Training}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Require:}}
\REQUIRE Initial success classifier $D(\vec{o}) \rightarrow [0, 1]$, positive examples $\mathcal{P} = \{ \text{interactable object(s)}\} $   %$\mathcal{P} = \{(\vec{s}, 1)\}$ %(interaction-ready states)
\jdtext{I wonder if we could clearly define ``actionable states'' e.g. it contains a latent unobserved state $s$, an unknown transition function $\mathcal{T}(s'|s, a)$, and an observation function $o(s)$. In other words, $P={s, \mathcal{T}(s'|s, a), o(s)}$. With that context we could say things about we have a collection of positives, etc. Otherwise this is likely to be a point of confusion.}.

%\jd{Notation needs fixing.}


% \STATE $\Pi^0 =  \operatorname*{argmax}_{\Pi} \E[\log( D(f(\vec{o}_{t+1} \mid \vec{s}_t, \Pi (\vec{a}_t \mid \vec{o}_t))))]$
\STATE Train an initial task policy with visual classifier reward in MDP $M_{task}$ \jdtext{Where is $p_\Pi$ defined?}
\begin{align}
    \Pi^0 =  \operatorname*{argmax}_{\Pi} \operatorname*{\E}_{\tau \sim p_{\Pi} (\tau)} \sum_{t = 1}^T \log( D(\vec{o}_{t} ))
\end{align}

\STATE Rollout $\vec{s}_T \sim p_{\Pi^0} (\tau)$ for $n$ times
\STATE Collect $n$ negative examples $\mathcal{D} \leftarrow \{(\vec{s}_T, 0)\}$ \jdtext{JD: Should this not also be an ``interactable'' negative state?}
\STATE Train a verification policy in MDP $M_{v}$, where the environment is initialized from $(\vec{s},l) \sim \mathcal{P} \cup \mathcal{D}$ \jdtext{Where is $f$ defined?}
\begin{align}
    \pi_{v} = \operatorname*{argmax}_{\pi_{v}} \bigg[ \operatorname*{\E}_{\vec{s} \sim \mathcal{P}} [\log (D(f(\vec{o}' \mid \vec{s}, \pi_{v} (\vec{a} \mid \vec{o}))))] + \operatorname*{\E}_{\vec{s} \sim \mathcal{D}} [\log (1 - D(f(\vec{o}' \mid \vec{s}, \pi_{v} (\vec{a} \mid \vec{o}))))] \bigg]
\label{eq:pi_v_rew}
\end{align}

\STATE Train a new task policy with the additional verification reward in MDP $M_{task}^*$
\begin{align}
    \Pi^{adv} =  \operatorname*{argmax}_{\Pi} & \bigg[ \operatorname*{\E}_{\tau \sim p_{\Pi} (\tau)} \sum_{t = 1}^T \log( D(\vec{o}_{t} )) 
    + \lambda \operatorname*{\E}_{\vec{s}_T \sim p_{\Pi} (\tau)} \log (D(f(\vec{o}' \mid \vec{s}_T, \pi_{v} (\vec{a} \mid \vec{o}_T)))) \bigg]
\label{eq:adv_pi_task_rew}
\end{align}

\end{algorithmic}
\label{algo:main_algo}
\end{algorithm}

